ManiCast: Collaborative Manipulation with Cost-Aware Human Forecasting

Seamless human-robot manipulation in close proximity relies on accurate forecasts of human motion. While there has been significant progress in learning forecast models at scale, when applied to manipulation tasks, these models accrue high errors at critical transition points leading to degradation in downstream planning performance. Our key insight is that instead of predicting the most likely human motion, it is sufficient to produce forecasts that capture how future human motion would affect the cost of a robot's plan. We present ManiCast, a novel framework that learns cost-aware human forecasts and feeds them to a model predictive control planner to execute collaborative manipulation tasks. Our framework enables fluid, real-time interactions between a human and a 7-DoF robot arm across a number of real-world tasks such as reactive stirring, object handovers, and collaborative table setting. We evaluate both the motion forecasts and the end-to-end forecaster-planner system against a range of learned and heuristic baselines while additionally contributing new datasets. We release our code and datasets at https://portal-cornell.github.io/manicast/.

==> introduction/introduction.tex <==
\section{Introduction}

==> paper/experiments/forecasting_table.tex <==
\begin{table}[t]
\centering
\resizebox{\textwidth}{!}
{
\begin{tabular}{ccccccccccc}
\toprule
& Models $\xrightarrow{}$  & \multicolumn{2}{c}{\textsc{Baselines}} && \multicolumn{6}{c}{\textsc{Learning-Based}}\\  \cmidrule{3-4} \cmidrule{6-11}
& Metrics (mm) $\downarrow$  & {\textsc{CUR}} & {\textsc{CVM}}  && {\textsc{Base}} & {\textsc{Scratch}} & {\textsc{FineTuned}} & {\textsc{ManiCast-T}} & {\textsc{ManiCast}} & {\textsc{ManiCast-W}}\\   
% & & ADE & FDE && ADE & FDE  && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE && ADE & FDE\\
\midrule
\parbox[t]{2}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{{AMASS}}}}}
&All Joints ADE & 102.5 (\pm 0.2) &194.9 (\pm 0.4) &&\tbcolorg 63.0 (\pm 0.1) &181.2 (\pm 0.2) &99.0 (\pm 0.1) &103.5 (\pm 0.1) &103.5 (\pm 0.1) &99.1 (\pm 0.1)\\
&All Joints FDE &120.6 (\pm 0.3) &333.6 (\pm 0.6) &&\tbcolorg 92.1 (\pm 0.2) &196.7 (\pm 0.2) &136.8 (\pm 0.2) &141.6 (\pm 0.2) &141.5 (\pm 0.2) &135.3 (\pm 0.2)\\
&Wrists ADE &182.9 (\pm 0.3) &353.7 (\pm 0.7) &&\tbcolorg 103.9 (\pm 0.2) &263.0 (\pm 0.3) &157.5 (\pm 0.3) &160.0 (\pm 0.3) &157.2 (\pm 0.3) &156.0 (\pm 0.3)\\
&Wrists FDE &211.0 (\pm 0.5) &602.5 (\pm 1.3) &&\tbcolorg 154.8 (\pm 0.4) &275.4 (\pm 0.4) &218.6 (\pm 0.4) &219.7 (\pm 0.4) &212.8 (\pm 0.4) &214.4 (\pm 0.4)\\
\midrule
\parbox[t]{2}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textsc{{ReactStir}}}}}
&All Joints ADE &63.0 (\pm 1.2) &84.3 (\pm 1.3) &&67.7 (\pm 1.0) &67.4 (\pm 0.9) &\tbcolorg 44.8 (\pm 0.7) &50.6 (\pm 0.6) &45.1 (\pm 0.6) &45.2 (\pm 0.6)\\
&All Joints FDE &103.2 (\pm 2.2) &166.4 (\pm 2.8) &&110.8 (\pm 2.0) &102.1 (\pm 1.7) &81.0 (\pm 1.6) &91.3 (\pm 1.5) &\tbcolorg 80.5 (\pm 1.5) &81.7 (\pm 1.5)\\
&Wrists ADE &83.6 (\pm 1.7) &116.2 (\pm 1.8) &&94.8 (\pm 1.4) &93.6 (\pm 1.3) &64.7 (\pm 1.1) &75.9 (\pm 1.0) &67.1 (\pm 1.0) &\tbcolorg 62.9 (\pm 1.0)\\
&Wrists FDE &136.9 (\pm 3.0) &225.6 (\pm 3.8) &&154.2 (\pm 2.8) &137.9 (\pm 2.3) &113.2 (\pm 2.3) &131.7 (\pm 2.1) &115.0 (\pm 2.2) &\tbcolorg 110.2 (\pm 2.1)\\
&T-Wrists ADE &132.7 (\pm 3.3) &166.9 (\pm 3.7) &&134.3 (\pm 3.3) &129.2 (\pm 2.7) &94.9 (\pm 2.4) &91.1 (\pm 2.1) &89.5 (\pm 2.2) &\tbcolorg 85.3 (\pm 2.1)\\
&T-Wrists FDE &226.1 (\pm 5.8) &334.7 (\pm 7.5) &&233.8 (\pm 6.0) &203.5 (\pm 4.9) &179.5 (\pm 4.9) &171.3 (\pm 4.4) &168.9 (\pm 4.6) &\tbcolorg 163.9 (\pm 4.5)\\
% &T-Wrists FDE &226.1 (\pm 5.8) &334.7 (\pm 7.5) &&233.8 (\pm 6.0) &203.5 (\pm 4.9) &179.5 (\pm 4.9) &171.3 (\pm 4.4) &168.9 (\pm 4.6) &\tbcolorg 163.9 (\pm 4.5)\\
% &T-Wrists FDE &226.1 (\pm 5.8) &334.7 (\pm 7.5) &&233.8 (\pm 6.0) &203.5 (\pm 4.9) &179.5 (\pm 4.9) &171.3 (\pm 4.4) &168.9 (\pm 4.6) &\tbcolorg 163.9 (\pm 4.5)\\
\midrule
\parbox[t]{2}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textsc{{Handover}}}}}
&All Joints ADE &38.9 (\pm 0.4) &57.1 (\pm 0.5) &&45.2 (\pm 0.3) &49.9 (\pm 0.3) &\tbcolorg31.8 (\pm 0.3) &34.1 (\pm 0.3) &32.5 (\pm 0.3) &32.4 (\pm 0.3)\\
&All Joints FDE &62.3 (\pm 0.7) &110.3 (\pm 1.1) &&70.4 (\pm 0.7) &68.3 (\pm 0.6) &\tbcolorg54.6 (\pm 0.6) &57.5 (\pm 0.6) &54.7 (\pm 0.6) &54.8 (\pm 0.6)\\
&Wrists ADE &55.1 (\pm 0.6) &84.3 (\pm 0.8) &&62.0 (\pm 0.5) &68.4 (\pm 0.5) &46.8 (\pm 0.5) &50.7 (\pm 0.4) &48.2 (\pm 0.4) &\tbcolorg45.8 (\pm 0.4)\\
&Wrists FDE &88.1 (\pm 1.1) &162.0 (\pm 1.6) &&100.1 (\pm 1.0) &92.6 (\pm 0.8) &79.0 (\pm 0.9) &84.5 (\pm 0.8) &79.4 (\pm 0.8) &\tbcolorg 77.2 (\pm 0.8)\\
&T-Wrists ADE &82.4 (\pm 1.3) &114.0 (\pm 1.6) &&84.8 (\pm 1.2) &91.2 (\pm 1.0) &67.6 (\pm 1.0) &64.8 (\pm 0.9) &65.8 (\pm 0.9) &\tbcolorg 62.6 (\pm 0.9)\\
&T-Wrists FDE &140.0 (\pm 2.2) &228.7 (\pm 3.5) &&146.7 (\pm 2.1) &130.7 (\pm 1.6) &124.5 (\pm 1.9) &118.3 (\pm 1.7) &118.7 (\pm 1.7) &\tbcolorg 113.4 (\pm 1.7)\\
\midrule
\parbox[t]{2}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{{TableSet}}}}}
&All Joints ADE &76.5 (\pm 1.1) &99.1 (\pm 1.3) &&80.4 (\pm 1.3) &90.2 (\pm 1.3) &58.6 (\pm 1.0) &57.6 (\pm 1.3) &\tbcolorg 53.6 (\pm 0.7) &56.1 (\pm 1.0)\\
&All Joints FDE &130.3 (\pm 1.9) &199.9 (\pm 2.9) &&137.7 (\pm 2.1) &134.3 (\pm 1.9) &110.5 (\pm 1.7) &106.7 (\pm 2.0) &\tbcolorg 101.7 (\pm 1.5) &105.1 (\pm 1.6)\\
&Wrists ADE &103.6 (\pm 1.5) &139.0 (\pm 1.7) &&107.3 (\pm 1.5) &114.8 (\pm 1.3) &82.5 (\pm 1.2) &79.6 (\pm 1.4) &76.7 (\pm 1.0) &\tbcolorg 74.8 (\pm 1.0)\\
&Wrists FDE &176.0 (\pm 2.5) &276.1 (\pm 3.7) &&185.5 (\pm 2.6) &165.0 (\pm 2.2) &151.1 (\pm 2.2) &143.1 (\pm 2.3) &140.9 (\pm 2.1) &\tbcolorg 138.8 (\pm 2.0)\\
\bottomrule

\end{tabular}
}

\vspace{3pt}
\caption{Average forecast metrics (in mm) for all models across all datasets.}
\vspace{-9mm}
\label{tab:forecasting_metrics}
\end{table}



==> paper/experiments/old_table.tex <==
\begin{table}[t]
\centering

% \vspace{3pt}
% \renewcoand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{
\begin{tabular}{
cccccccccccccc}
\toprule
& Model \xrightarrow{}  & \multicolumn{2}{c}{\textsc{GroundTruth}} && \multicolumn{2}{c}{\textsc{Baselines}} && \multicolumn{6}{c}{\textsc{Learning-Based}}\\ \cmidrule{9-14} \cmidrule{3-4} \cmidrule{6-7}
& Metric \downarrow & \textsc{Cur} & \textsc{Fut} && \textsc{CV} & \textsc{Worst} && \textsc{Base} & \textsc{FT-only} & \textsc{FT} & \textsc{FT-T-only} & \textsc{FT-T-mixed} & \textsc{FT-TJ}\\ 
% \vspace{2}
 % \hline
 
\midrule
\parbox[t]{2}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{AMASS}}}} 

 & MPJPE (mm) & 102 & 0 && 195 & - && \tbcolorg 63 & 181 & 99 & 104 & 103 & \tbcolorg 99\\ 
 & FDE (mm) & \tbcolorg 121 & 0 && 334 & - && \tbcolorg 92 & 196 & 137 & 142 & 141 & 135\\
  & Wrist-ADE (mm) & 183 & 0 && 354 & - && \tbcolorg 104 & 263 & 158 & 160 & 157 & \tbcolorg 156\\
  & Wrist-FDE (mm) & \tbcolorg 211 & 0 && 602 & - && \tbcolorg 155 & 276 & 219 & 220 & 212 & 214\\

% \vspace{2pt}  
\midrule
% \hline
\parbox[t]{2}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textsc{Reactive Stirring}}}}
& MPJPE (mm) & 63 & 0 && 84 & - && 68 & 67 & \tbcolorg 45 & 51 & \tbcolorg 45 & \tbcolorg 45\\
 & FDE (mm) & 103 & 0 && 166 & - && 110 & 102 & \tbcolorg 81 & 91 & \tbcolorg 81 & 82\\
  & Wrist-ADE (mm) & 84 & 0 && 116 & - && 95 & 94 & \tbcolorg 65 & 76 & 67 & \tbcolorg 63\\
  & Wrist-FDE (mm) & 137 & 0 && 226 & - && 154 & 138 & \tbcolorg 113 & 132 & 114 & \tbcolorg 110\\
  & T-Wrist ADE (mm) & 211 & 0 && 166 & - && 134 & 129 &  95 & 91 & \tbcolorg 89 & \tbcolorg 86\\
  & T-Wrist FDE (mm) & 226 & 0 && 335 & - && 234 & 203 & 180 & 171 & \tbcolorg 168 & \tbcolorg 164\\
 & Stop Time (ms) & 0 & 1000 && \tbcolorg 368 & \tbcolorg 1000 && -139 & -238 & 203 & \tbcolorg 271 & 247 & \tbcolorg 290\\
 & Restart Time (ms) & 0 & 1000 && 236 & 0 && 257 & 235 & 441 & \tbcolorg 454 & \tbcolorg 456 & \tbcolorg 497\\
  & FDR & \tbcolorg 0\% & 0\% && 67\% & 100\% && 11\% & 11\% & \tbcolorg 0\% & 11\% & \tbcolorg 0\% & 11\%\\
\midrule
% \hline
\parbox[t]{2}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textsc{Object Handover}}}}
 & MPJPE (mm) & 39 & 0 && 57 & - && 45 & 49 & \tbcolorg 32 & 34 & \tbcolorg 32 & \tbcolorg 32\\
 & FDE (mm) & 62 & 0 && 110 & - && 70 & 68 & \tbcolorg 55 & 58 & \tbcolorg 54 & \tbcolorg 55\\
  & Wrist-ADE (mm) & 56 & 0 && 84 & - && 62 & 68 & \tbcolorg 46 & 50 & 48 & \tbcolorg 46\\
  & Wrist-FDE (mm) & 88 & 0 && 162 & - && 100 & 92 & \tbcolorg 79 & 84 & 80 & \tbcolorg 77\\
  & T-Wrist ADE (mm) & 83 & 0 && 114 & - && 84 & 92 &  68 & \tbcolorg 64 & 66 & \tbcolorg 62\\
  & T-Wrist FDE (mm) & 140 & 0 && 228 & - && 146 & 131 & 124 & \tbcolorg 118 & \tbcolorg 118 & \tbcolorg 114\\
  & Goal Detection (ms) & 0 & 1000 &&  246& - &&  -127 & -62 & 189 & \tbcolorg 473 &  450 & \tbcolorg 488\\
  & Correct Goal Rate & \tbcolorg 100\% & 100\% && 20\% & 0\% && 90\% & 80\% & \tbcolorg 100\% & \tbcolorg 100\% & \tbcolorg 100\% & \tbcolorg 100\%\\
  & Path Length (mm) &  459 & 381 && 485 & - && 489 & 466 &  432 & \tbcolorg 428 & \tbcolorg 404& 436\\
  & Time to Goal (s)& 4.59 & 2.87 && 3.77 & - && 4.32 & 4.60 & \tbcolorg 3.87 & \tbcolorg 3.91 &  3.96& 4.17\\
\midrule
% \hline

\parbox[t]{2}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{SetTable}}}}
 & MPJPE (mm) & 76 & 0 && 99 & - && 80 & 90 & 59 & 58 & \tbcolorg 54 & \tbcolorg 56\\
 & FDE (mm) & 130 & 0 && 200 & - && 138 & 134 & 111 & 107 & \tbcolorg 102 & \tbcolorg 105\\
  & Wrist-ADE (mm) & 104 & 0 && 139 & - && 108 & 114 & 82 & 80 & \tbcolorg 76 & \tbcolorg 74\\
  & Wrist-FDE (mm) & 176 & 0 && 276 & - && 186 & 165 & 151 & 143 & \tbcolorg 140 & \tbcolorg 139\\
% \midrule
\bottomrule

\end{tabular}
}
\label{table:tabletop_metrics}
\vspace{3pt}
\caption{Results for forecasting and three manipulation tasks with different models.}
\end{table}

==> related_work/related_work.tex <==
\section{Related Work}

\input{related_work/human_motion}

==> report/embodiment.tex <==
\section{Human to Robot Embodiment}

In this work, we first train a human motion predictor $P_\psi(\xi_{-i} | \xi_i, \phi)$ and then use a planner that optimizes the cost function $C(\xi_i, \xi_{-i})$. The input to this motion predictor is the joint positions of the humans in the scene. However, when deployed with our robotic arm, we will have to match the robot representation with the human. This might be trivially achieved by defined a modified version of the collision avoidance component in the cost function. However, we still have to consider the learned forecasting model. We can make the following modifications:

\begin{enumerate}
    \item \textbf{Match Arm Markers: } We can redefine the forecasting problem to focus on reaching arm motion, similar to \cite{Mainprice2015PredictingHR}. In this case, we will consider the forecasting problem to focus on just one arm. Each arm acts as a separate agent in the scene. This should be relatively simple to modify in the existing forecasting model architectures. We would simply select just 4 markers (the pelvis, shoulder, elbow and wrist) to represent an arm.
    \item \textbf{Simplified Geometric Representation: } When predicting forecasts, we can incorporate information about the other agents in the scene via simplified geometrical objects. Specifically, we represent each human arm as two cylinders (between the wrist, elbow and the elbow, shoulder). This would requires restructuring the existing forecasting models to consume the modified inputs.
\end{enumerate}

==> report/human_motion.tex <==
\section{Human Motion Forecasting}

\textbf{IOC + Planning: }\citet{Mainprice2015PredictingHR} predict single-arm reaching motion (only upper body human data) using motion capture of two humans performing a collaborative task in a shared workspace. They first learn weights for a collision avoidance cost function that best explains the collected human-human data using Inverse Optimal Control (IOC). The collision avoidance cost functions consists of 16 pairwise distance functions between 4 joints (i.e, the wrist, elbow, shoulder, and pelvis). Then, to predict human motion, the authors utilize the STOMP motion planning algorithm to replan paths for each human iteratively such that it best explains the learned cost function. However, the planner does not directly utilize the predictions of the other human. This work also requires the kinematic tree to explain human dynamics, which requires manual labeling of the joint interactions within the human. Further, the forecasting model relies on just 7 collected trajectories. Recently, large databases of human motion have been released. We exploit this data for building reliable forecasting models in this work.

\textbf{Single-Human Motion Forecasting: }The AMASS (Archive of Motion Capture As Surface Shapes) \cite{AMASS:ICCV:2019} is a large and varied database of human motion that unifies 15 different optical marker-based mocap datasets by representing them within a common framework and parameterization. It consists of more than 40 hours of single-human motion spanning over 300 different subjects. \citet{Mao2020HistoryRI} note that human motion over a time horizon is smooth and periodic. They exploit this observation by encoding the context of an agent with a Discrete Cosine Transform (DCT) and then apply an attention module to capture the similarities between current and historical motion sub-sequences, allowing the model to aggregate past motions for long-term prediction. STS-GCN \cite{Sofianos2021SpaceTimeSeparableGC} learn the adjacency matrix between different joints and across different timesteps seperately to bottleneck the cross-talk interactions between the joints across time. Then, they use a Temporal Convolutional Network (TCN) for decoding the human motion predictions over a fixed time horizon.

\textbf{Multi-Human Motion Forecasting: } Recently, multiple datasets of multi-human motion have been open-sourced. This includes the 3D Poses in the Wild Dataset (3DPW) \cite{vonMarcard2018} which contains over 60 annoted human motion video sequences in realworld settings which each scene containing 2-3 humans. Some works that produce socially aware human motion predictions are listed down:
\begin{enumerate}
    \item SoMoFormer: Multi-Person Pose Forecasting with Transformers \cite{Vendrow2022SoMoFormerMP}
    \item Multi-Person 3D Motion Prediction with Multi-Range Transformers \cite{Wang2021MultiPerson3M}
    \item TRiPOD: Human Trajectory and Pose Dynamics Forecasting in the Wild \cite{Adeli2021TRiPODHT}
\end{enumerate}
The first approach relies on masking out the future trajectory of the human and using the transformer to fill out the mask. Modifying this approach would allow us to develop a conditional forecasting model.




==> report/planner.tex <==
\section{Planner}

To solve the planning problem, we can utilize the following classes of approaches:

\begin{itemize}
    \item \textbf{Sampling-Based MPC}: STORM \cite{Bhardwaj2021FastJS} is a state of the art sampling-based MPC planner. It gives us access to a sampler that provides us an elite distribution of plans, which can be used to train the forecaster.
    \item \textbf{Optimal Control} : FrankaPy \cite{zhang2020modular} provides implementation of optimal control algorithms like LQR on the Franka Panda ARM. If our cost function can be quadraticized in terms of the robot state, we can also access gradients through the planner.
    \item \textbf{SBMP using Potential Functions:} MoveIt!\cite{Coleman2014ReducingTB} provides implementations of various OMPL \cite{Sucan2012TheOM} SBMPs like RRT*, PRM*, etc. that can plan paths from a start configuration to a goal configuration representing the human arm as an obstacle using potential functions.
\end{itemize}



==> report/planning_with_humans.tex <==
\section{Planning Alongside Humans}

We want robots to plan alongside humans.

Usually robots come to a stop when a human comes in the workspace

Otherwise you create simple approximations of how a human would approach the workspace.

==> report/problem_formulation.tex <==
\section{Problem Formulation}

\textbf{Forecasting: }We model the forecasting problem as a multi-agent Contextual Markov Decision Process (CMDP). A state for each agent at timestep $t$ is represented by $s_t^{i} \in \mathbb{R}^{J\times3}$ which consists of the 3D coordinates of $J$ joints for each agent. The combined state of all N agents in the scene can be represented by $S_t = \{s_t^{0}, s_t^{1}, \dots, s_t^{N}\}$. Let $\phi = \{S_0, S_1, \dots, S_t\}$ denote the context -- a history of past states for all the agents in the current scene. The future trajectories for the humans in the scene is represented by $\xi = \{S_{t+1}, S_{t+2}, \dots, S_{t+T}\}$ For each agent, we aim to learn a conditional distribution over future trajectories of the other agents in the scene using $P_\psi(\xi_{-1} | \xi_i, \phi)$, where $\psi$ are the learnt model parameters.

\textbf{Cost Function: } We define a cost function for an agent's trajectory by $C(\xi_i | \xi_{-1}) : \mathbb{R}^{N \times T \times J \times 3} \rightarrow \mathbb{R}$. This cost function is composed of three components:
\begin{enumerate}
    \item Goal-Reaching Component $G(\xi_i): $ This represents the component of the cost function that favors proximity of the trajectory to the intended goal of the agent's task.
    \item Collision Avoidance Component $D(\xi_i | \xi_{-i}): $ This component penalizes an agent's trajectory for being close to the other agents in the scene.
    \item Smoothness Component $A(\xi):$ This term enforces smoothness (i.e., control cost) of the agent trajectory.
\end{enumerate}


\textbf{Planner: } The planner attempts to find a trajectory for each agent that minimizes the above cost function:
\begin{equation}
    \label{eq:nominal_planning}
    \argmin_{\xi_i} \; \underset{\substack{\hat{\xi}_{-i} \sim P_\theta(.|\xi_i, \phi)}}{\mathbb{E}} C({\xi}_i | \hat{\xi}_{-i})
\end{equation}
Note that only the collision avoidance component of the cost function requires access to the trajectories of the other agents, $\xi_{-i}$, in the scene. At the current timestep, an agent does not directly have access to the future motion. Instead, it relies on the forecasting model to provide estimated motion of the other agents in the scene, $\hat{\xi}_{-i} \sim P_\psi(. | \xi_i, \phi)$.


